Front-end Electronics for Timing with pico-seconds precision using 3D Trench Silicon Sensors

The next generation of collider experiments require tracking detectors with extreme performance capabilities in terms of spatial resolution (tens of $\mu \text{m}$), radiation hardness ($10^{17}~1~$MeV n$_{eq}/$cm$^2$) and timing resolution (tens of ps). 3D silicon sensors, recently developed within the TimeSPOT initiative, offer a viable solution to cope with such demanding requirements. In order to accurately characterize the timing performance of these new sensors, several read-out boards, based on discrete active components, have been designed, assembled, and tested. The same electronics is also suitable for characterization of similar pixel sensors whenever timing performance in the order and below 10 ps is a requirement. This paper describes the general characteristics needed by front-end electronics to exploit solid-state sensors with fast timing capabilities and in particular, showcases the performance of the developed electronics in the testing and characterization of fast 3D silicon sensors.

==> bib.tex <==
@article{JINST-TimeSpot,
	doi = "10.3389/fnins.2013.12345",
	URL = "http://www.frontiersin.org/Journal/10.3389/fnins.2013.12345/abstract",
	author =" Lucio Anderlini and Aresti, M. and Bizzeti,A. and Boscardin, M. and Cardini, A. and Dalla Betta, G.-F. and Ferrero, M. and Forcolin, G. and Garau, M. and Lai, A. and Lampis, A. and Loi, A. and Lucarelli, C. and Mendicino, R. and Mulargia, R. and Obertino, M. and Robutti, E. and Ronchin, S. and Ruspa, M. and Vecchi, S.",
	title ="{Intrinsic time resolution of 3D-trench silicon pixels for charged particle detection}", 
	journal ="{Journal of Instrumentation}",
	volume = "15",
	pages = "P09029",
	year = "{2020}"
}
@article{LAI2020164491,
title = {{First results of the TIMESPOT project on developments on fast sensors for future vertex detectors}},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {981},
pages = {164491},
month = nov,
year = {2020},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2020.164491},
author = "Lai, A. and others",
}

@article{3Dstepper,
author = "Boscardin, M. and others",
year = {2021},
month = {01},
pages = {},
title = {Advances in 3D Sensor Technology by Using Stepper Lithography},
volume = {8},
journal = {Frontiers in Physics},
doi = {10.3389/fphy.2020.625275}
}

@article{Ferrero_2020,
	Abstract = {The recent development in the design of Ultra Fast Silicon Detector (UFSD), aimed at combining radiation resistance up to fluences of 1015 neq/cm2 and fine read-out segmentation, makes these sensors suitable for high energy physics applications. UFSD is an evolution of standard silicon sensor, optimized to achieve excellent timing resolution (∼30 ps), thanks to an internal low gain (∼20). UFSD sensors are n in p Low Gain Avalanche Diode (LGAD) with an active thickness of ∼5 μm. The internal gain in LGAD is obtained by implanting an appropriate density of acceptors (of the order of ∼ 1016/cm3) close to the p-n junction, that, when depleted, locally generates an electric field high enough to activate the avalanche multiplication; this layer of acceptors is called gain layer. The two challenges in the development of UFSD for high energy physics detectors are the radiation hardness and the fine segmentation of large area sensors. Irradiation fluences of the order of 1015 neq/cm2 have a dramatic effect on the UFSD: neutrons and charged hadrons reduce the active acceptor density forming the gain layer; this mechanism, called initial acceptor removal, causes the complete disappearance of the internal gain above fluence of 1015 neq/ cm2. For the segmentation of UFSDs, the crucial point is the electrical insulation of pads and the extension of the inactive area between pads. In this paper we present the latest results on radiation resistance of LGADs with different gain layer designs, irradiated up to 3⋅1015 neq/ cm2. Three different segmentation technologies, developed by Fondazione Bruno Kessler in Trento, will also be discussed in detail in the second part of the paper.},
	author = "Ferrero, M. and others",
	Doi = {10.1088/1748-0221/15/04/c04027},
	Journal = {Journal of Instrumentation},
	Month = {apr},
	Number = {04},
	Pages = {C04027--C04027},
	Publisher = {{IOP} Publishing},
	Title = {Evolution of the design of ultra fast silicon detector to cope with high irradiation fluences and fine segmentation},
	Url = {https://doi.org/10.1088/1748-0221/15/04/c04027},
	Volume = {15},
	Year = 2020,
	Bdsk-Url-1 = {https://doi.org/10.1088/1748-0221/15/04/c04027},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/1748-0221/15/04/c04027}}

@article{Iacobucci_2022,
	Abstract = {A monolithic silicon pixel detector prototype has been produced in the SiGe BiCMOS SG13G2 130 nm node technology by IHP. The ASIC contains a matrix of hexagonal pixels with pitch of approximately 100 μm. Three analog pixels were calibrated in laboratory with radioactive sources and tested in a 180 GeV/c pion beamline at the CERN SPS. A detection efficiency of (99.9-0.2 +0.1)% was measured together with a time resolution of (36.4 $\pm$ 0.8) ps at the highest preamplifier bias current working point of 150 μA and at a sensor bias voltage of 160 V. The ASIC was also characterized at lower bias voltage and preamplifier current.},
	author = "Iacobucci, G. and others",
	Doi = {10.1088/1748-0221/17/02/p02019},
	Journal = {Journal of Instrumentation},
	Month = {feb},
	Number = {02},
	Pages = {P02019},
	Publisher = {{IOP} Publishing},
	Title = {Efficiency and time resolution of monolithic silicon pixel detectors in {SiGe} {BiCMOS} technology},
	Url = {https://doi.org/10.1088/1748-0221/17/02/p02019},
	Volume = {17},
	Year = 2022,
	Bdsk-Url-1 = {https://doi.org/10.1088/1748-0221/17/02/p02019},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/1748-0221/17/02/p02019}}
}

@article{3D-accurate,
   title={{Accurate modelling of 3D-trench silicon sensor with enhanced timing performance and comparison with test beam measurements}},
   volume={16},
   ISSN={1748-0221},
   DOI={10.1088/1748-0221/16/09/p09028},
   number={09},
   journal=JINST,
   publisher={IOP Publishing},
   author={Brundu, D. and Cardini, A. and Contu, A. and Cossu, G.M. and Dalla Betta, G.-F. and Garau, M. and Lai, A. and Lampis, A. and Loi, A. and Obertino, M.M. and Siddi, G.B. and Vecchi, S.},
   year={2021},
   month=sep,
   pages={P09028}
}

@article{Minafra_2020,
	Abstract = {Timing detectors are a well-established part of High Energy Physics experimental instrumentation. The choice of sensors with fast (less than 10 ns) and precise (better than 100 ps) signals, together with radiation resistance considerations, are an essential part of the design of a timing detector. In this paper, the main characteristics that make single diamond crystal sensors ideal for timing applications will be described and an introduction to the design of fast front-end electronics will be given. Finally, two examples of diamond timing detectors used in High Energy Physics, the START detector of HADES and the TOTEM/CMS timing detector, will be discussed.},
	Author = {Bossini, Edoardo and Minafra, Nicola},
	Doi = {10.3389/fphy.2020.00248},
	Issn = {2296-424X},
	Journal = {Frontiers in Physics},
	Title = {Diamond Detectors for Timing Measurements in High Energy Physics},
	Url = {https://www.frontiersin.org/article/10.3389/fphy.2020.00248},
	Volume = {8},
	Year = {2020},
	Bdsk-Url-1 = {https://www.frontiersin.org/article/10.3389/fphy.2020.00248},
	Bdsk-Url-2 = {http://dx.doi.org/10.3389/fphy.2020.00248}}


@article{Berretti_2017,
	Abstract = {This paper describes the performance of a prototype timing detector, based on 50 μm thick Ultra Fast Silicon Detector, as measured in a beam test using a 180 GeV/c momentum pion beam. The dependence of the time precision on the pixel capacitance and bias voltage is investigated in this paper. A timing precision from 30 ps to 100 ps (RMS), depending on the pixel capacitance, has been measured at a bias voltage of 180 V.},
	Author = {M. Berretti and R. Arcidiacono and E. Bossini and M. Bozzo and N. Cartiglia and M. Ferrero and V. Georgiev and T. Isidori and R. Linhart and N. Minafra and M.M. Obertino and V. Sola and N. Turini},
	Doi = {10.1088/1748-0221/12/03/p03024},
	Journal = {Journal of Instrumentation},
	Month = {mar},
	Number = {03},
	Pages = {P03024--P03024},
	Publisher = {{IOP} Publishing},
	Title = {Test of Ultra Fast Silicon Detectors for the {TOTEM} upgrade project},
	Url = {https://doi.org/10.1088/1748-0221/12/03/p03024},
	Volume = {12},
	Year = 2017,
	Bdsk-Url-1 = {https://doi.org/10.1088/1748-0221/12/03/p03024},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/1748-0221/12/03/p03024}}

@article{CARTIGLIA201783,
	Abstract = {In this paper we report on the timing resolution obtained in a beam test with pions of 180GeV/c momentum at CERN for the first production of 45µm thick Ultra-Fast Silicon Detectors (UFSD). UFSD are based on the Low-Gain Avalanche Detector (LGAD) design, employing n-on-p silicon sensors with internal charge multiplication due to the presence of a thin, low-resistivity diffusion layer below the junction. The UFSD used in this test had a pad area of 1.7mm2. The gain was measured to vary between 5 and 70 depending on the sensor bias voltage. The experimental setup included three UFSD and a fast trigger consisting of a quartz bar readout by a SiPM. The timing resolution was determined by doing Gaussian fits to the time-of-flight of the particles between one or more UFSD and the trigger counter. For a single UFSD the resolution was measured to be 34ps for a bias voltage of 200V, and 27ps for a bias voltage of 230V. For the combination of 3 UFSD the timing resolution was 20ps for a bias voltage of 200V, and 16ps for a bias voltage of 230V.},
	author = "Cartiglia, N. and others",
	Doi = {https://doi.org/10.1016/j.nima.2017.01.021},
	Issn = {0168-9002},
	Journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
	Keywords = {Fast silicon sensors, Charge multiplication, Thin tracking sensors, Silicon strip, Pixel detectors},
	Pages = {83-88},
	Title = {Beam test results of a 16ps timing system based on ultra-fast silicon detectors},
	Url = {https://www.sciencedirect.com/science/article/pii/S0168900217300219},
	Volume = {850},
	Year = {2017},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0168900217300219},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.nima.2017.01.021}}



@misc{UCSC,
    author = "{UCSC board Twiki page}",
    title = {https://twiki.cern.ch/twiki/bin/view/Main/UcscSingleChannel},
    year          = "2020"
}


@article{RiassuntoEUStrat,
author = {Aleksa, M. and others},
title = "{Strategic RD Programme on Technologies for Future Experiments}", 
journal ="Tech. Rep. CERN-OPEN-2018-006, CERN, Geneva",
year ={2018},
url = "https://cds.cern.ch/record/2649646"
}

@misc{timespot,
    author = "{TimeSPOT collaboration}",
    title = {web site: https://web.infn.it/timespot/index.php},
    year          = "2020"
}

@techreport{bib:FTDRLHCbU2,
      author        = {{The LHCb Collaboration}},
      title         = "{Framework TDR for the LHCb Upgrade II: Opportunities in flavour physics, and beyond, in the HL-LHC era}",
      institution   = "CERN",
      address       = "Geneva",
      reportNumber  = "CERN/LHCC-2021-012",
      month         = "Feb",
      year          = "2022",
      url           = "https://cds.cern.ch/record/2776420/files/LHCB-TDR-023.pdf",
}

@article{Ramo,
author = "{Ramo, S.}", 
title = "{Currents Induced by Electron Motion}",
doi = {10.1109/JRPROC.1939.228757},
journal={Proceedings of the IRE, vol. 27, no. 9, pp. 584-585},
year ={1939}
}

@article{3D,
author = "Parker, S. and others",
title = "{3D- A proposed new architecture for solid-state radiation detectors}",
journal ={NIM A395, 328-34},
year = {1997}
}

@article{LaiCossu,
  doi = {10.48550/ARXIV.2008.09867},
  url = {https://arxiv.org/abs/2008.09867},
  author = {Lai, Adriano and Cossu, Gian Matteo},
  keywords = {Instrumentation and Detectors (physics.ins-det), High Energy Physics - Experiment (hep-ex), FOS: Physical sciences, FOS: Physical sciences},
  title = "{High-resolution timing electronics for fast pixel sensors}",
  journal = "{arXiv2008.09867}",
  year = {2020},
  copyright = {Creative Commons Attribution 4.0 International},
}

@INPROCEEDINGS{LabMeas,
  author={Aresti, Mauro and Cardini, Alessandro and Lai, Adriano and Loi, Angelo and Cossu, Gian Matteo and Garau, Michela and Lampis, Andrea and Betta, Gian-Franco Dalla and Forcolin, Giulio},
  booktitle={2020 IEEE Nuclear Science Symposium and Medical Imaging Conference (NSS/MIC)}, 
  title="{Laboratory Characterization of Innovative 3D trench-design Silicon Pixel Sensors Using a Sub-Picosecond Precision Laser-Based Testing Equipment}", 
  year={2020},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/NSS/MIC42677.2020.9507747},
  }
  
  @INPROCEEDINGS{Laser,
  author={Aresti, Mauro and Cardini, Alessandro and Cossu, Gian Matteo and Garau, Michela and Lai, Adriano and Lampis, Andrea and Loi, Angelo},
  booktitle={2020 IEEE Nuclear Science Symposium and Medical Imaging Conference (NSS/MIC)}, 
  title="{A Sub-Picosecond Precision Laser-Based Test Station for The Measurement of Silicon Detector Timing Performances}", 
  year={2020},
  volume={},
  number={},
  pages={1-4},
  doi={10.1109/NSS/MIC42677.2020.9507743},
  }


@article{TFboost,
	Abstract = {Particle tracking for future experiments at colliders is an incredible challenge in terms of sensor technology and readout. Simulation tools are a crucial ingredient to investigate new layouts able to cope with harsh radiation conditions and, at the same time, provide valuable timing information for track finding algorithms. Detailed and numerous simulations of energy deposits as well as sensor and front-end electronics responses imply a heavy usage of computing resources. In this paper, we present two software packages that, via massive parallelization and dedicated algorithms, allow for a significant speed-up in simulation time.},
	Author = {Brundu, D. and Contu, A. and Cossu, G. M. and Loi, A.},
	Doi = {10.3389/fphy.2022.804752},
	Issn = {2296-424X},
	Journal = {Frontiers in Physics},
	Title = "{Modeling of Solid State Detectors Using Advanced Multi-Threading: The TCoDe and TFBoost Simulation Packages}",
	Url = {https://www.frontiersin.org/article/10.3389/fphy.2022.804752},
	Volume = {10},
	Year = {2022},
	Bdsk-Url-1 = {https://www.frontiersin.org/article/10.3389/fphy.2022.804752},
	Bdsk-Url-2 = {http://dx.doi.org/10.3389/fphy.2022.804752},
	}

@article{Parker,
author ="{Parker, S.I. and Kok A., and Kenney C. and Jarron P. and Hasi J. and Despeisse M. and Da Via C. and Anelli G.}",
title = "{Increased speed: 3D silicon sensors; fast current amplifiers}",
  journal={IEEE Trans. Nucl. Sci., 58 (2), pp. 404-417},
  year={2011}
}

@misc{MichelaTrento,
author = {Michela Garau},
title = "{Laboratory characterization of 3D-trench silicon pixel sensors with a 90Sr radioactive source}",
note = "Talk given at the 16th Trento Workshop On Advanced Silicon Radiation Detectors",
year= {2021},
url = "{https://indico.cern.ch/event/983068/contributions/4223212/}"
}



@misc{AndreaTrento,
author = {Andrea Lampis},
title = "{Sub-pixel characterization of innovative 3D trench-design silicon pixel sensors using ultra-fast laser-based testing equipment}",
note = "Talk given at the 16th Trento Workshop On Advanced Silicon Radiation Detectors",
year= {2021},
url = "{https://indico.cern.ch/event/983068/contributions/4223202/}"
}

@misc{CardiniPisa,
author = {Alessandro Cardini},
title = "{10 ps timing with 3D trench 
silicon pixel sensors}",
note = "Talk given at the 15th Pisa Meeting on Advanced Detector",
year= {2022},
url = "{https://agenda.infn.it/event/22092/contributions/167338/attachments/91326/124025/TimeSPOT_Elba2022%20Final.pdf}"
}

@misc{Andreaiworid,
author = {Andrea Lampis},
title = "{10 ps timing with 3D trench 
silicon pixel sensors}",
note = "Talk given at the 23rd International Workshop on Radiation Imaging Detectors",
year= {2022},
url = "{https://indico.cern.ch/event/1120714/contributions/4867208/attachments/2472539/4242526/Andrea_Lampis_iworid2022.pdf}"
}

@article{SADROZINSKI,
title = "{Ultra-fast silicon detectors (UFSD)}",
journal = "Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment",
volume = "831",
pages = "18 - 23",
year = "2016",
note = "Proceedings of the 10th International “Hiroshima” Symposium on the Development and Application of Semiconductor Tracking Detectors",
issn = "0168-9002",
doi = "https://doi.org/10.1016/j.nima.2016.03.093",
url = "http://www.sciencedirect.com/science/article/pii/S0168900216301279",
author = "H.F.-W. Sadrozinski and others",
keywords = "Fast silicon sensors, Charge multiplication, Thin tracking sensors, Silicon strip, Pixel detectors",
abstract = "We report on measurements on Ultra-Fast Silicon Detectors (UFSD) which are based on Low-Gain Avalanche Detectors (LGAD). They are n-on-p sensors with internal charge multiplication due to the presence of a thin, low-resistivity diffusion layer below the junction, obtained with a highly doped implant. We have performed several beam tests with LGAD of different gain and report the measured timing resolution, comparing it with laser injection and simulations. For the 300μm thick LGAD, the timing resolution measured at test beams is 120ps while it is 57ps for IR laser, in agreement with simulations using Weightfield2. For the development of thin sensors and their readout electronics, we focused on the understanding of the pulse shapes and point out the pivotal role the sensor capacitance plays."
}

@article{3Dradhard,
author = "Manna, M.  and others",
title = "{First characterization of 3D pixel detectors irradiated at extreme fluences}",
journal = "NIM-A",
volume  = "979",
year    = "2020"
}

@misc{tcad,
author = "{{Synopsys Inc.}}",
title  = "{Synopsys Sentaurus TCAD Version 2018.06 K-2015.06}", 
year = {2018},
url = {https://www.synopsys.com/silicon/tcad.html},
}

@book{Razavi,
author = "Behzad Razavi",
title = "{Design of Integrated Circuits for Optical communications}", 
publisher = "John Wiley \& Sons", 
year = "2012",
}

@misc{infineon,
author = "{{Infineon Technologies}}",
title = "{Ultra low-noise Si-Ge:C transistors for use up to 12 Ghz}",
year = {2022},
url = "{https://www.infineon.com/}",
}

@incollection{Bosch,
title = "{Chapter 21 - Deep Reactive Ion Etching}",
editor = "Markku Tilli and Teruaki Motooka and Veli-Matti Airaksinen and Sami Franssila and Mervi Paulasto-Kröckel and Veikko Lindroos",
booktitle = "Handbook of Silicon Based MEMS Materials and Technologies (Second Edition)",
publisher = "William Andrew Publishing",
edition = "Second Edition",
address = "Boston",
pages = "444 - 469",
year = "2015",
series = "Micro and Nano Technologies",
isbn = "978-0-323-29965-7",
doi = "https://doi.org/10.1016/B978-0-323-29965-7.00021-X",
url = "http://www.sciencedirect.com/science/article/pii/B978032329965700021X",
author = "Franz Laermer and Sami Franssila and Lauri Sainiemi and Kai Kolari",
keywords = "Reactive ion etching, deep reactive ion etching, Bosch process, cryo-process, photoresist mask, notching effect, scalloping",
abstract = "This chapter discusses reactive ion etching and deep reactive ion etching on wafers detailing the various equipment and reactor requirements for different applications. The Bosch process is explained in detail as is cryogenic DRIE with details on the various etch masks for silicon. The issues and challenges of DRIE, such as vertical and sloped sidewalls, loading effect, lag, scalloping, notching effect are covered. This chapter also discusses the applications of DRIE such as free shape structures, small feature sizes, high aspect ratios, and deep and multidepth structures, as well as the post-DRIE etch treatments. The factors favoring either wet or dry etching are briefly given."
}

@article{ATLAS-IBL,
author = "Abbot, B. and others",
title = "{Production and integration of the ATLAS Insertable B-Layer}",
journal = "JINST",
volume  = "13",
year    = "2018",
pages = "T05008",
doi = "10.1088/1748-0221/13/05/t05008"
}

@article{ATLAS-IBL2,
author = "Da Via, C. and others",
title = "{3D silicon sensors:Design, large area production and quality assurance for ATLASIBL pixel detector upgrade}",
journal = "CERN-LHCC-2017-021 ; ATLAS-TDR-030",
year    = "2017"
}

@article{ATLAS-ITk,
author = "{ATLAS collaboration}",
title = "{Technical Design Report for the ATLAS Inner Tracker Pixel Detector}",
journal = "CERN-LHCC-2017-021 ; ATLAS-TDR-030",
year    = "2017"
}

@misc{Timepix4,
    author = {X. Llopart},
    title = "{The design of the Timepix4 chip: a 230 kpixel and 4-side buttable chip with 200ps on-pixel time bin resolution and 15-bits of TOT energy resolution}",
    url = "https://indico.cern.ch/event/788037/attachments/1946069/3233311/Xavi_Timepix4_ESE.pdf",
  year    = "{https://indico.cern.ch/event/788037/attachments/1946069/3233311/Xavi\_Timepix4\_ESE.pdf, 2019}"
}


@article{Loi_2021,
	Abstract = {Solid state sensors having timing capabilities below 50 ps RMS are becoming a mandatory requirement in particle tracking techniques of future experiments at colliders. Within this context, silicon sensors with 3D structure provide an interesting solution, due to their intrinsic fast response and radiation resistance. The performance of such devices is strictly dependent on the geometric structure of the electrodes and can be considerably optimised by design using suitable tools to accurately model the sensor behaviour. This paper illustrates the development, performance and use of the TCoDe simulator, specifically dedicated to the fast simulation of carrier transportation phenomena in solid state sensors. Some examples of its effectiveness in the design and analysis of 3D sensors are also given.},
	Author = {A. Loi and A. Contu and A. Lai},
	Doi = {10.1088/1748-0221/16/02/p02011},
	Journal = {Journal of Instrumentation},
	Month = {feb},
	Number = {02},
	Pages = {P02011--P02011},
	Publisher = {{IOP} Publishing},
	Title = {Timing optimisation and analysis in the design of 3D silicon sensors: the {TCoDe} simulator},
	Url = {https://doi.org/10.1088/1748-0221/16/02/p02011},
	Volume = {16},
	Year = 2021,
	Bdsk-Url-1 = {https://doi.org/10.1088/1748-0221/16/02/p02011},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/1748-0221/16/02/p02011}}
}


@misc{tcode,
  author       = {Contu, A. and Loi, A.},
  title        = "{MultithreadCorner/TCode}",
  doi          = {10.5281/zenodo.3686010},
  url          = {https://doi.org/10.5281/zenodo.3686010},
  year    = "2020"
}

@misc{hydra,
  author       = {Alves Junior, A.A.},
  title        = "{MultithreadCorner/Hydra}",
  doi          = {10.5281/zenodo.1206261},
  url          = {https://doi.org/10.5281/zenodo.1206261},
  year    = "2020"
}

@misc{root,
  title        = "{https://root.cern}",
  year    = "2020"
}

@article{Geant4,
     author    = "Agostinelli, S. and others", 
     collaboration = "{{Geant4 collaboration}}",
     title     = "{Geant4: A simulation toolkit}",
     journal   = "Nucl. Instrum. Meth.",
     volume    = "A506",
     year      = "2003",
     pages     = "250",
     doi       = "10.1016/S0168-9002(03)01368-8"
}

@article{Riegler,
	doi = {10.1088/1748-0221/12/11/p11017},
	url = {https://doi.org/10.1088%2F1748-0221%2F12%2F11%2Fp11017},
	year = 2017,
	month = {nov},
	publisher = {{IOP} Publishing},
	journal = {Journal of Instrumentation},
	volume = {12},
	number = {11},
	pages = {P11017--P11017},
	author = {W. Riegler and G. Aglieri Rinella},
	title = {Time resolution of silicon pixel sensors},
	abstract = {We derive expressions for the time resolution of silicon   detectors, using the Landau theory and a PAI model for describing   the charge deposit of high energy particles. First we use the   centroid time of the induced signal and derive analytic expressions   for the three components contributing to the time resolution, namely   charge deposit fluctuations, noise and fluctuations of the signal   shape due to weighting field variations. Then we derive expressions   for the time resolution using leading edge discrimination of the   signal for various electronics shaping times. Time resolution of   silicon detectors with internal gain is discussed as well.}
}

@book{blum2008particle,
  title={Particle Detection with Drift Chambers},
  author={Blum, W. and Riegler, W. and Rolandi, L.},
  isbn={9783540766841},
  lccn={2007940836},
  series={Particle Acceleration and Detection},
  url={https://books.google.it/books?id=RgxUlAXv0RAC},
  year={2008},
  publisher={Springer Berlin Heidelberg}
}


@article{Benoit2016100,
	author = {Benoit, M. and Cardarelli, R. and D{\' e}bieux, S. and Favre, Y. and Iacobucci, G. and Nessi, M. and Paolozzi, L. and Shu, K.},
	journal = {Journal of Instrumentation},
	number = {3},
	year = {2016},
	month = {mar 9},
	title = {100 ps time resolution with thin silicon pixel detectors and a {SiGe} {HBT} amplifier - {IOPscience}},
	howpublished = {https://iopscience.iop.org/article/10.1088/1748-0221/11/03/P03011},
	volume = {11},
}


@unpublished{forcolin,
title= {Development of 3D Trenched-Electrode 
Pixel Sensors with Improved Timing 
performance},
author = {G. Forcolin},
year = {2019},
note= {Hiroshima Symposium 2019},
URL= {https://indico.cern.ch/event/803258/contributions/3582928/attachments/1962456/3262167/337-Forcolin-HiroshimaTimespotV3.pdf},
}

@techreport{FTDR,
      author        = "LHCb Collaboration, CERN (Meyrin)",
      title         = "{Framework TDR for the LHCb Upgrade II $\text{-
                       Opportunities in flavour physics, and beyond, in the HL-LHC
                       era} $}",
      institution   = "CERN",
      reportNumber  = "CERN-LHCC-2021-012, LHCB-TDR-023",
      address       = "Geneva",
      year          = "2021",
      url           = "https://cds.cern.ch/record/2776420",
}

@ARTICLE{adriano_last,
  
AUTHOR={Lai, Adriano},   
	 
TITLE={4D-tracking in the 10-ps range: A technological perspective},      
	
JOURNAL={Frontiers in Physics},      
	
VOLUME={10},           
	
YEAR={2022},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fphy.2022.1019262},       
	
DOI={10.3389/fphy.2022.1019262},      
	
ISSN={2296-424X},   
   
ABSTRACT={The present paper focuses on recent and ready-to-come advancements concerning high-resolution 4D-tracking with a perspective approach. Four-dimensional-tracking techniques (particle tracking with timing information for each detection point) have revealed a necessity for the next and next-to-next generations of high-energy physics experiments to cope with the increasing luminosity and consequent event pile-up in the beam collision region. Such a decisive challenge concerns both detection and processing technologies at an unprecedented level of difficulty. In addition to the high performance required in space–time measurement precision (some tens of picoseconds resolution in timing and about 10 µm resolution in space), an extremely high radiation hardness is demanded for such technologies together with an extremely high read-out and processing capability. Emerging experimental solutions for sensors and electronics against such challenges are presented here.}
}

@article{Piccolo_2022,
	doi = {10.1088/1748-0221/17/03/c03022},
  
	url = {https://doi.org/10.1088%2F1748-0221%2F17%2F03%2Fc03022},
  
	year = 2022,
	month = {mar},
  
	publisher = {{IOP} Publishing},
  
	volume = {17},
  
	number = {03},
  
	pages = {C03022},
  
	author = {L. Piccolo and S. Cadeddu and L. Frontini and A. Lai and V. Liberali and A. Rivetti and A. Stabile},
  
	title = {First measurements on the Timespot1 {ASIC}: a fast-timing, high-rate pixel-matrix front-end},
  
	journal = {Journal of Instrumentation}
}
